Composed Variational Natural Language Generation for Few-shot Intents

In this paper, we focus on generating training examples for few-shot intents in the realistic imbalanced scenario. To build connections between existing many-shot intents and few-shot intents, we consider an intent as a combination of a domain and an action, and propose a composed variational natural language generator (CLANG), a transformer-based conditional variational autoencoder. CLANG utilizes two latent variables to represent the utterances corresponding to two different independent parts (domain and action) in the intent, and the latent variables are composed together to generate natural examples. Additionally, to improve the generator learning, we adopt the contrastive regularization loss that contrasts the in-class with the out-of-class utterance generation given the intent. To evaluate the quality of the generated utterances, experiments are conducted on the generalized few-shot intent detection task. Empirical results show that our proposed model achieves state-of-the-art performances on two real-world intent detection datasets.

==> 2problem_defination.tex <==
\section{Problem Formulation}
We first define intent in this section, then formally state the problem.

\noindent\textbf{Intent.} An intent is a purpose, or a goal that underlies user input utterance \cite{ibm2017doc}. When users interact with intelligent assistants, they intent to get some information or execute a command in a certain domain, such as ask about the weather or process a bill payment. In this paper, we define the intent structurally with a domain and an action. For example, an intent of asking about the weather has the action of ``Query'' and is in the domain of ``Weather''. Formally, we denote the domain as $y_d$ and the action as $y_a$. Each intent can be expressed as a pair of $y = (y_d, y_a)$.

give an utterance as a example.

We therefore define an intent as a text phrase
consisting of two parts: (i) an action, which is a word or phrase
representing a tangible purpose, task or activity which is to be
requested or performed, and (ii) an object, which represents those
entity words or phrases that the action is going to act or operate
upon \cite{vedula2019towards}

We observe from the previous illustrations that the Action
component of an intent is likely to consist of a verb or infinitive
phrase that follows a noun or a subject phrase. Further, the Object
component of an intent often comprises of a noun or compound
noun (i.e., an expression with multiple nouns) phrase, possibly
qualified by adverbs or adjectives.

These include previously unseen intent typesthat were not encountered while training, unlike a classifier that
helps us understand novel intents

\noindent\textbf{Generalized Few-shot Intent Detection.} Given an existing intent set ${\mathcal Y_{ex}}$ with sufficient labeled examples $\mathcal D_{ex} = \{(x_i, y_i), i = 1, 2, ..., |\mathcal{D}_{ex}|\}$ with $y_i \in {\mathcal Y_{ex}}$. The novel intent set set can be denoted as $\mathcal{Y}_{novel}$, where each intent has $K$ examples $\mathcal D_{novel} = \bigcup_{n}\{(x_{n,k}, y_n)\}_{k=1}^K$. $K$ is a small number such as 1 or 5. These two intent sets are disjointed, i.e., $\mathcal Y_{ex} {\cap}  \mathcal Y_{novel}=\varnothing$; the overall intent space can be denoted as $\mathcal Y_{joint} = \mathcal Y_{ex} \cup \mathcal Y_{novel}$.

Generalized few-shot intent detection intends to classify a given utterance in the joint label space consisting not only the xisting intents but also the novel intents. Formally, given a new query utterance $x$, the GFSID task aims at inferring the the most likely intent of $x$, i.e.,
$\hat{y} = \mathop {\arg \max }\limits_{y \in {\mathcal Y_{joint}}} p\left( {y|x, \mathcal D_{ex}, \mathcal D_{novel}} \right).$

